Mixing and de-mixing of model microswimmers in bi-motility mixtures

Cooperation between micro-organisms give rise to novel phenomena like clustering, swarming in suspension. We study the collective behavior of the artificial swimmer called Taylor line at low Reynolds number using multi-particle collision dynamics method. In this paper we have modeled bi-motility mixtures of multiple swimmers in 2 dimensions, which differ from each other by the velocity with which they swim. We observe that the swimmers can segregate into slower and faster ones depending on the relative difference in velocity of the 2 type of swimmers. We also observe that contribution of slower swimmers towards clustering, on an average, is much larger compared to faster ones, although we employ a homogeneous mixture. When the difference in velocity is large between the swimmers, the faster ones move away from the slower ones towards the boundary. On the other hand, when the relative difference in velocity is very small, the slower and faster swimmer mix together to form big clusters. At later time even for small difference in velocity the swimmers segregate into fast and slow swimmer clusters.

==> refer <==
@suppcollection{suppl,
note = {See Supplemental Material at [URL will be inserted by publisher] for further information}
}
@article{Ramaswamy2017,
abstract = {The study of systems with sustained energy uptake and dissipation at the scale of the constituent particles is an area of central interest in nonequilibrium statistical physics. Identifying such systems as a distinct category -- Active Matter -- unifies our understanding of autonomous collective move- ment in the living world and in some surprising inanimate imitations. In this article I present the Active Matter framework, briefly recall some early work, review our recent results on single-particle and collective behaviour, including experiments on active granular monolayers, and discuss new directions for the future.},
archivePrefix = {arXiv},
arxivId = {1705.06269},
author = {Ramaswamy, Sriram},
doi = {10.1088/1742-5468/aa6bc5},
eprint = {1705.06269},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1705.06269.pdf:pdf},
issn = {1742-5468},
title = {{Active matter}},
url = {http://arxiv.org/abs/1705.06269{\%}0Ahttp://dx.doi.org/10.1088/1742-5468/aa6bc5},
year = {2017}
}
@article{Ponisch2017,
author = {P{\"{o}}nisch, Wolfram and Weber, Christoph A and Juckeland, Guido and Biais, Nicolas and Zaburdaev, Vasily},
doi = {10.1088/1367-2630/aa5483},
issn = {13672630},
journal = {New J. Phys.},
keywords = {Neisseria gonorrhoeae,bacterial mechanics,biofilms,cell aggregation,multicellular phenomena},
month = {jan},
number = {1},
pages = {015003},
title = {{Multiscale modeling of bacterial colonies: How pili mediate the dynamics of single cells and cellular aggregates}},
url = {http://stacks.iop.org/1367-2630/19/i=1/a=015003?key=crossref.28c221a0d5a6820a77b2673c23babbe7},
volume = {19},
year = {2017}
}
@article{Malgaretti2017,
abstract = {We study different types of microswimmers moving in channels with varying cross section and thereby interacting hydrodynamically with the channel walls. Starting from the Smoluchowski equation for a dilute suspension, for which interactions among swimmers can be neglected, we derive analytic expressions for the lateral probability distribution between plane channel walls. For weakly corrugated channels we extend the Fick--Jacobs approach to microswimmers and thereby derive an effective equation for the probability distribution along the channel axis. Two regimes arise dominated either by entropic forces due to the geometrical confinement or by the active motion. In particular, our results show that the accumulation of microswimmers at channel walls is sensitive to both, the underlying swimming mechanism and the geometry of the channels. Finally, for asymmetric channel corrugation our model predicts a rectification of microswimmers along the channel, the strength and direction of which strongly depends on the swimmer type.},
archivePrefix = {arXiv},
arxivId = {1704.03170},
author = {Malgaretti, Paolo and Stark, Holger},
doi = {10.1063/1.4981886},
eprint = {1704.03170},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1704.03170.pdf:pdf},
issn = {00219606},
journal = {J. Chem. Phys.},
number = {17},
pages = {1--18},
title = {{Model microswimmers in channels with varying cross section}},
volume = {146},
year = {2017}
}
@article{Ariel2017,
abstract = {We describe a new mechanism for L{\'{e}}vy walks, explaining the recently observed superdiffusion of swarming bacteria. The model hinges on several key physical properties of bacteria, such as an elongated cell shape, self-propulsion, and a collectively generated regular vortexlike flow. In particular, chaos and L{\'{e}}vy walking are a consequence of group dynamics. The model explains how cells can fine-tune the geometric properties of their trajectories. Experiments confirm the spectrum of these patterns in fluorescently labeled swarming Bacillus subtilis.},
author = {Ariel, Gil and Be'Er, Avraham and Reynolds, Andy},
doi = {10.1103/PhysRevLett.118.228102},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.118.228102.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {22},
pages = {1--6},
title = {{Chaotic Model for L{\'{e}}vy Walks in Swarming Bacteria}},
volume = {118},
year = {2017}
}
@article{Li2017,
abstract = {Bacterial swimming in confined two-dimensional environments is ubiquitous in nature and in clinical settings. Characterizing individual interactions between swimming bacteria in 2D confinement will help to understand diverse microbial processes, such as bacterial swarming and biofilm formation. Here we report a novel motion pattern displayed by flagellated bacteria in 2D confinement: When two nearby cells align their moving directions, they tend to engage in cohesive swimming without direct cell body contact, as a result of hydrodynamic interaction but not flagellar intertwining. We further found that cells in cohesive swimming move with higher directional persistence, which can increase the effective diffusivity of cells by ∼3 times as predicted by computational modeling. As a conserved behavior for peritrichously flagellated bacteria, cohesive swimming in 2D confinement may be key to collective motion and self-organization in bacterial swarms; it may also promote bacterial dispersal in unsaturated soils and in interstitial space during infections.},
author = {Li, Ye and Zhai, He and Sanchez, Sandra and Kearns, Daniel B and Wu, Yilin},
doi = {10.1103/PhysRevLett.119.018101},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.119.018101.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jul},
number = {1},
pages = {018101},
title = {{Noncontact Cohesive Swimming of Bacteria in Two-Dimensional Liquid Films}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.119.018101 http://link.aps.org/doi/10.1103/PhysRevLett.119.018101},
volume = {119},
year = {2017}
}
@article{Junot2017,
abstract = {We experimentally study the mechanical pressure exerted by a set of respectively passive isotropic and self-propelled polar disks onto two different flexible unidimensional membranes. In the case of the isotropic disks, the mechanical pressure, inferred from the shape of the membrane, is identical for both membranes and follows the equilibrium equation of state of hard disks. On the contrary, for the self-propelled disks, the mechanical pressure strongly depends on the membrane in use and is thus not a state variable. When self propelled disks are present on both sides of the membrane, we observe an instability of the membrane akin to the one predicted theoretically for Active Brownian Particles against a soft wall. In that case, the integrated mechanical pressure difference across the membrane depends explicitly on the packing fraction on both sides, and does not reduce to a dependance on the sole packing fraction difference; a further evidence of the absence of equation of state.},
archivePrefix = {arXiv},
arxivId = {1703.04195},
author = {Junot, G. and Briand, G. and Ledesma-Alonso, R. and Dauchot, O.},
doi = {10.1103/PhysRevLett.119.028002},
eprint = {1703.04195},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.119.028002.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
keywords = {Experiment,Pressure},
month = {jul},
number = {2},
pages = {028002},
title = {{Active versus Passive Hard Disks against a Membrane: Mechanical Pressure and Instability}},
url = {http://arxiv.org/abs/1703.04195 http://link.aps.org/doi/10.1103/PhysRevLett.119.028002},
volume = {119},
year = {2017}
}
@article{Stenhammar2017,
abstract = {In this Letter, we study the collective behaviour of a large number of self-propelled microswimmers immersed in a fluid. Using unprecedently large-scale lattice Boltzmann simulations, we reproduce the transition to bacterial turbulence. We show that, even well below the transition, swimmers move in a correlated fashion that cannot be described by a mean-field approach. We develop a novel kinetic theory that captures these correlations and is non-perturbative in the swimmer density. To provide an experimentally accessible measure of correlations, we calculate the diffusivity of passive tracers and reveal its non-trivial density dependence. The theory is in quantitative agreement with the lattice Boltzmann simulations and captures the asymmetry between pusher and puller swimmers below the transition to turbulence.},
archivePrefix = {arXiv},
arxivId = {1703.01892},
author = {Stenhammar, Joakim and Nardini, Cesare and Nash, Rupert W. and Marenduzzo, Davide and Morozov, Alexander},
doi = {10.1103/PhysRevLett.119.028005},
eprint = {1703.01892},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.119.028005.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jul},
number = {2},
pages = {028005},
title = {{Role of Correlations in the Collective Behavior of Microswimmer Suspensions}},
url = {http://arxiv.org/abs/1703.01892 http://link.aps.org/doi/10.1103/PhysRevLett.119.028005},
volume = {119},
year = {2017}
}
@article{Smrek2017,
abstract = {Recent theoretical studies found that mixtures of active and passive colloidal particles phase separate but only at very high activity ratio. The high value poses serious obstacles for experimental exploration of this phenomenon. Here we show using simulations that when the active and passive particles are polymers, the critical activity ratio decreases with the polymer length. This not only facilitates the experiments but also has implications on the DNA organization in living cell nuclei. Entropy production can be used as an accurate indicator of this non-equilibrium phase transition.},
archivePrefix = {arXiv},
arxivId = {1701.07362},
author = {Smrek, Jan and Kremer, Kurt},
doi = {10.1103/PhysRevLett.118.098002},
eprint = {1701.07362},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.118.098002.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {9},
pages = {1--5},
title = {{Small Activity Differences Drive Phase Separation in Active-Passive Polymer Mixtures}},
volume = {118},
year = {2017}
}
@article{Ilkanaiv2017,
abstract = {Swarming bacteria collectively migrate on surfaces using flagella, forming dynamic whirls and jets that consist of millions of individuals. Because some swarming bacteria elongate prior to actual motion, cell aspect ratio may play a significant role in the collective dynamics. Extensive research on self-propelled rodlike particles confirms that elongation promotes alignment, strongly affecting the dynamics. Here, we study experimentally the collective dynamics of variants of swarming Bacillus subtilis that differ in length. We show that the swarming statistics depends on the aspect ratio in a critical, fundamental fashion not predicted by theory. The fastest motion was obtained for the wild-type and variants that are similar in length. However, shorter and longer cells exhibit anomalous, non-Gaussian statistics and nonexponential decay of the autocorrelation function, indicating lower collective motility. These results suggest that the robust mechanisms to maintain aspect ratios may be important for efficient swarming motility. Wild-type cells are optimal in this sense.},
author = {Ilkanaiv, Bella and Kearns, Daniel B. and Ariel, Gil and Beer, Avraham},
doi = {10.1103/PhysRevLett.118.158002},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.118.158002.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {15},
pages = {1--5},
title = {{Effect of Cell Aspect Ratio on Swarming Bacteria}},
volume = {118},
year = {2017}
}
@article{Blaschke2016,
author = {Blaschke, Johannes and Maurer, Maurice and Menon, Karthik and Z{\"{o}}ttl, Andreas and Stark, Holger},
doi = {10.1039/C6SM02042A},
issn = {1744-683X},
journal = {Soft Matter},
number = {48},
pages = {9821--9831},
title = {{Phase separation and coexistence of hydrodynamically interacting microswimmers}},
url = {http://xlink.rsc.org/?DOI=C6SM02042A},
volume = {12},
year = {2016}
}
@article{Zottl2016,
abstract = {Active colloids are microscopic particles, which self-propel through viscous fluids by converting energy extracted from their environment into directed motion. We first explain how articial microswimmers move forward by generating near-surface flow fields via self-phoresis or the self-induced Marangoni effect. We then discuss generic features of the dynamics of single active colloids in bulk and in confinement, as well as in the presence of gravity, field gradients, and fluid flow. In the third part, we review the emergent collective behavior of active colloidal suspensions focussing on their structural and dynamic properties. After summarizing experimental observations, we give an overview on the progress in modeling collectively moving active colloids. While active Brownian particles are heavily used to study collective dynamics on large scales, more advanced methods are necessary to explore the importance of hydrodynamic and phoretic particle interactions. Finally, the relevant physical approaches to quantify the emergent collective behavior are presented.},
archivePrefix = {arXiv},
arxivId = {1601.06643},
author = {Z{\"{o}}ttl, Andreas and Stark, Holger},
doi = {10.1088/0953-8984/28/25/253001},
eprint = {1601.06643},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Z{\"{o}}ttl{\_}2016{\_}J.{\_}Phys.{\%}3A{\_}Condens.{\_}Matter{\_}28{\_}253001.pdf:pdf},
issn = {0953-8984},
journal = {J. Phys. Condens. Matter},
keywords = {active colloids,collective motion,emergent behavior,in colour only in,some figures may appear,the online journal},
month = {jun},
number = {25},
pages = {253001},
pmid = {27171563},
title = {{Emergent behavior in active colloids}},
url = {http://arxiv.org/abs/1601.06643 http://stacks.iop.org/0953-8984/28/i=25/a=253001?key=crossref.4f31c1a4927a885005054f0c7ca05d87},
volume = {28},
year = {2016}
}
@article{Menzel2016,
abstract = {Dynamical density functional theory (DDFT) has been successfully derived and applied to describe on one hand passive colloidal suspensions, including hydrodynamic interactions between individual particles. On the other hand, active "dry" crowds of self-propelled particles have been characterized using DDFT. Here, we go one essential step further and combine these two approaches. We establish a DDFT for active microswimmer suspensions. For this purpose, simple minimal model microswimmers are introduced. These microswimmers self-propel by setting the surrounding fluid into motion. They hydrodynamically interact with each other through their actively self-induced fluid flows and via the common "passive" hydrodynamic interactions. An effective soft steric repulsion is also taken into account. We derive the DDFT starting from common statistical approaches. Our DDFT is then tested and applied by characterizing a suspension of microswimmers, the motion of which is restricted to a plane within a three-dimensional bulk fluid. Moreover, the swimmers are confined by a radially symmetric trapping potential. In certain parameter ranges, we find rotational symmetry breaking in combination with the formation of a "hydrodynamic pumping state," which has previously been observed in the literature as a result of particle-based simulations. An additional instability of this pumping state is revealed.},
archivePrefix = {arXiv},
arxivId = {1510.07593},
author = {Menzel, Andreas M. and Saha, Arnab and Hoell, Christian and L{\"{o}}wen, Hartmut},
doi = {10.1063/1.4939630},
eprint = {1510.07593},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/The Journal of Chemical Physics Volume 144 issue 2 2016 [doi 10.1063{\%}2F1.4939630] Menzel, Andreas M.$\backslash$; Saha, Arnab$\backslash$; Hoell, Christian$\backslash$; L{\"{o}}wen, Hartm -- Dynamical density functional theory for microswimme.pdf:pdf},
issn = {1089-7690},
journal = {J. Chem. Phys.},
month = {jan},
number = {2},
pages = {024115},
pmid = {26772562},
title = {{Dynamical density functional theory for microswimmers.}},
url = {http://arxiv.org/abs/1510.07593 http://dx.doi.org/10.1063/1.4939630 http://www.ncbi.nlm.nih.gov/pubmed/26772562},
volume = {144},
year = {2016}
}
@article{Ryan2016,
abstract = {Simultaneous acquisition of phase-contrast light microscopy and fluorescently labeled bacteria, moving within a dense swarm, reveals the intricate interactions between cells and the collective flow around them. By comparing wild-type and immotile cells embedded in a dense wild-type swarm, the effect of the active thrust generated by the flagella can be singled out. It is shown that while the distribution of angles among cell velocity, cell orientation, and the local flow around it is Gaussian-like for immotile bacteria, wild-type cells exhibit anomalous non-Gaussian deviations and are able to move in trajectories perpendicular to the collective flow. Thus, cells can maneuver or switch between local streams and jets. A minimal model describing bacteria as hydrodynamic force dipoles shows that steric effects, hydrodynamics interactions, and local alignments all have to be taken into account to explain the observed dynamics. These findings shed light on the physical mechanisms underlying bacterial swarming and the balance between individual and collective dynamics.},
author = {Ryan, Shawn D. and Ariel, Gil and Be'er, Avraham},
doi = {10.1016/j.bpj.2016.05.043},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1-s2.0-S0006349516303903-main.pdf:pdf},
issn = {15420086},
journal = {Biophys. J.},
number = {1},
pages = {247--255},
pmid = {27410751},
publisher = {Biophysical Society},
title = {{Anomalous Fluctuations in the Orientation and Velocity of Swarming Bacteria}},
url = {http://dx.doi.org/10.1016/j.bpj.2016.05.043},
volume = {111},
year = {2016}
}
@article{Weber2016,
author = {Weber, Simon N. and Weber, Christoph A. and Frey, Erwin},
doi = {10.1103/PhysRevLett.116.058301},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/Binary Mixtures of Particles with Diﬀerent Diﬀusivities Demix S Weber.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {5},
pages = {058301},
title = {{Binary Mixtures of Particles with Different Diffusivities Demix}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.058301},
volume = {116},
year = {2016}
}
@article{Theers2016,
abstract = {The friction and diffusion coefficients of rigid spherical colloidal particles dissolved in a fluid are determined from velocity and force autocorrelation functions by mesoscale hydrodynamic simulations. Colloids with both slip and no-slip boundary conditions are considered, which are embedded in fluids modelled by multiparticle collision dynamics (MPC) with and without angular momentum conservation. For no-slip boundary conditions, hydrodynamics yields the well-known Stokes law, while for slip boundary conditions the lack of angular momentum conservation leads to a reduction of the hydrodynamic friction coefficient compared to the classical result. The colloid diffusion coefficient is determined by integration of the velocity autocorrelation function, where the numerical result at shorter times is combined with the theoretical hydrodynamic expression for longer times. The suitability of this approach is confirmed by simulations of sedimenting colloids. In general, we find only minor deviations from the Stokes-Einstein relation, which even disappear for larger colloids. Importantly, for colloids with slip boundary conditions, our simulation results contradict the frequently assumed additivity of local and hydrodynamic diffusion coefficients.},
archivePrefix = {arXiv},
arxivId = {arXiv:1603.02888v1},
author = {Theers, Mario and Westphal, Elmar and Gompper, Gerhard and Winkler, Roland G.},
doi = {10.1103/PhysRevE.93.032604},
eprint = {arXiv:1603.02888v1},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/MPCD hydrodynamic friction in Brownian motion Mario Theers.pdf:pdf},
issn = {15502376},
journal = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
number = {3},
pages = {1--13},
pmid = {27078411},
title = {{From local to hydrodynamic friction in Brownian motion: A multiparticle collision dynamics simulation study}},
volume = {93},
year = {2016}
}
@article{Li2016,
abstract = {We study the collective motion of a suspension of rodlike microswimmers in a two-dimensional film of viscoelastic fluids. We find that the fluid elasticity has a small effect on a suspension of pullers, while it significantly affects the pushers. The attraction and orientational ordering of the pushers are enhanced in viscoelastic fluids. The induced polymer stresses break down the large-scale flow structures and suppress velocity fluctuations. In addition, the energy spectra and induced mixing in the suspension of pushers are greatly modified by fluid elasticity.},
author = {Li, Gaojin and Ardekani, Arezoo M.},
doi = {10.1103/PhysRevLett.117.118001},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/PhysRevLett.117.118001.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {11},
pages = {1--5},
title = {{Collective Motion of Microorganisms in a Viscoelastic Fluid}},
volume = {117},
year = {2016}
}
@article{Munch2016,
abstract = {Microorganisms naturally move in microstructured fluids. Using the simulation method of multi-particle collision dynamics, we study an undulatory Taylor line swimming in a two-dimensional microchannel and in a cubic lattice of obstacles, which represent simple forms of a microstructured environment. In the microchannel the Taylor line swims at an acute angle along a channel wall with a clearly enhanced swimming speed due to hydrodynamic interactions with the bounding wall. While in a dilute obstacle lattice swimming speed is also enhanced, a dense obstacle lattice gives rise to geometric swimming. This new type of swimming is characterized by a drastically increased swimming speed. Since the Taylor line has to fit into the free space of the obstacle lattice, the swimming speed is close to the phase velocity of the bending wave traveling along the Taylor line. While adjusting its swimming motion within the lattice, the Taylor line chooses a specific swimming direction, which we classify by a lattice vector. When plotting the swimming velocity versus the magnitude of the lattice vector, all our data collapse on a single master curve. Finally, we also report more complex trajectories within the obstacle lattice.},
archivePrefix = {arXiv},
arxivId = {1604.02408},
author = {M{\"{u}}nch, Jan L. and Alizadehrad, Davod and Babu, Sujin B. and Stark, Holger},
doi = {10.1039/C6SM01304J},
eprint = {1604.02408},
file = {:C$\backslash$:/Users/Adyant/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\"{u}}nch et al. - 2016 - Taylor line swimming in microchannels and cubic lattices of obstacles.pdf:pdf},
issn = {1744-683X},
journal = {Soft Matter},
number = {35},
pages = {7350--7363},
pmid = {27510576},
title = {{Taylor line swimming in microchannels and cubic lattices of obstacles}},
url = {http://xlink.rsc.org/?DOI=C6SM01304J},
volume = {12},
year = {2016}
}
@article{Hu2015a,
author = {Hu, Jinglei and Yang, Mingcheng and Gompper, Gerhard and Winkler, Roland G.},
doi = {10.1039/C5SM01678A},
issn = {1744-683X},
journal = {Soft Matter},
number = {40},
pages = {7867--7876},
title = {{Modelling the mechanics and hydrodynamics of swimming E. coli}},
url = {http://xlink.rsc.org/?DOI=C5SM01678A},
volume = {11},
year = {2015}
}
@article{Benisty2015,
abstract = {Under sublethal antibiotics concentrations, the statistics of collectively swarming Bacillus subtilis transitions from normal to anomalous, with a heavy-tailed speed distribution and a two-step temporal correlation of velocities. The transition is due to changes in the properties of the bacterial motion and the formation of a motility-defective subpopulation that self-segregates into regions. As a result, both the colonial expansion and the growth rate are not affected by antibiotics. This phenomenon suggests a new strategy bacteria employ to fight antibiotic stress.},
author = {Benisty, Sivan and Ben-Jacob, Eshel and Ariel, Gil and Be'er, Avraham},
doi = {10.1103/PhysRevLett.114.018105},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.114.018105.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {1},
pages = {1--5},
pmid = {25615508},
title = {{Antibiotic-induced anomalous statistics of collective bacterial swarming}},
volume = {114},
year = {2015}
}
@article{Stenhammar2015,
abstract = {We investigate the phase behavior and kinetics of a mixture of active ($\backslash$textit{\{}i.e.{\}}, self-propelled) and passive isometric Brownian particles through Brownian dynamics simulations and theory. As in a purely active system, motility of the active component triggers phase separation into a dense and a dilute phase; in the dense phase we further find active-passive segregation, with "rafts" of passive particles in a "sea" of active particles. We find that phase separation from an initially disordered mixture can occur with as little as 15 percent of the particles being active. Finally, we show that a system prepared in a suitable fully segregated initial state reproducibly self-assembles an active "corona" which triggers crystallization of the passive core by initiating a compression wave. Our findings are relevant to the experimental pursuit of directed self-assembly using active particles.},
archivePrefix = {arXiv},
arxivId = {1408.5175},
author = {Stenhammar, Joakim and Wittkowski, Raphael and Marenduzzo, Davide and Cates, Michael E.},
doi = {10.1103/PhysRevLett.114.018301},
eprint = {1408.5175},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.114.018301.pdf:pdf},
isbn = {0031-9007},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {1},
pages = {1--5},
pmid = {25615509},
title = {{Activity-induced phase separation and self-assembly in mixtures of active and passive particles}},
volume = {114},
year = {2015}
}
@article{Weitz2015,
abstract = {We study collections of self-propelled rods (SPR) moving in two dimensions for packing fractions less than or equal to 0.3. We find that in the thermodynamical limit the SPR undergo a phase transition between a disordered gas and a novel phase-separated system state. Interestingly, (global) orientational order patterns -- contrary to what has been suggested -- vanish in this limit. In the found novel state, the SPR self-organize into a highly dynamical, high-density, compact region - which we call aggregate - which is surrounded by a disordered gas. Active stresses build inside aggregates as result of the combined effect of local orientational order and active forces. This leads to the most distinctive feature of these aggregates: constant ejection of polar clusters of SPR. This novel phase-separated state represents a novel state of matter characterized by large fluctuations in volume and shape, related to mass ejection, and exhibits positional as well as orientational local order. SPR systems display new physics unseen in other active matter systems due to the coupling between density, active stresses, and orientational order (such coupling cannot be reduced simply to a coupling between speed and density).},
archivePrefix = {arXiv},
arxivId = {1507.00948},
author = {Weitz, Sebastian and Deutsch, Andreas and Peruani, Fernando},
doi = {10.1103/PhysRevE.92.012322},
eprint = {1507.00948},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevE.92.012322.pdf:pdf},
issn = {15502376},
journal = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
number = {1},
pages = {1--9},
title = {{Self-propelled rods exhibit a phase-separated state characterized by the presence of active stresses and the ejection of polar clusters}},
volume = {92},
year = {2015}
}
@article{Elgeti2014,
abstract = {Locomotion and transport of microorganisms in fluids is an essential aspect of life. Search for food, orientation toward light, spreading of off-spring, and the formation of colonies are only possible due to locomotion. Swimming at the microscale occurs at low Reynolds numbers, where fluid friction and viscosity dominates over inertia. Here, evolution achieved propulsion mechanisms, which overcome and even exploit drag. Prominent propulsion mechanisms are rotating helical flagella, exploited by many bacteria, and snake-like or whip-like motion of eukaryotic flagella, utilized by sperm and algae. For artificial microswimmers, alternative concepts to convert chemical energy or heat into directed motion can be employed, which are potentially more efficient. The dynamics of microswimmers comprises many facets, which are all required to achieve locomotion. In this article, we review the physics of locomotion of biological and synthetic microswimmers, and the collective behavior of their assemblies. Starting from individual microswimmers, we describe the various propulsion mechanism of biological and synthetic systems and address the hydrodynamic aspects of swimming. This comprises synchronization and the concerted beating of flagella and cilia. In addition, the swimming behavior next to surfaces is examined. Finally, collective and cooperate phenomena of various types of isotropic and anisotropic swimmers with and without hydrodynamic interactions are discussed.},
archivePrefix = {arXiv},
arxivId = {1412.2692},
author = {Elgeti, Jens and Winkler, Roland G. and Gompper, Gerhard},
doi = {10.1088/0034-4885/78/5/056601},
eprint = {1412.2692},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/[I]Physics of microswimmers{\_}single particle motion and collective behavior.pdf:pdf},
isbn = {0034-4885},
issn = {0034-4885},
journal = {Reports Prog. Phys.},
month = {may},
number = {5},
pages = {056601},
pmid = {25919479},
publisher = {IOP Publishing},
title = {{Physics of microswimmers—single particle motion and collective behavior: a review}},
url = {http://arxiv.org/abs/1412.2692{\%}0Ahttp://dx.doi.org/10.1088/0034-4885/78/5/056601 http://stacks.iop.org/0034-4885/78/i=5/a=056601?key=crossref.098e1dfca7db8f1f68a5a86fca9219b5},
volume = {78},
year = {2015}
}
@article{Hu2015,
abstract = {Bacteria such as Escherichia coli swim along circular trajectories adjacent to surfaces. Thereby, the orientation (clockwise, counterclockwise) and the curvature depend on the surface properties. We employ mesoscale hydrodynamic simulations of a mechano-elastic model of E. coli, with a spherocylindrical body propelled by a bundle of rotating helical flagella, to study quantitatively the curvature of the appearing circular trajectories. We demonstrate that the cell is sensitive to nanoscale changes in the surface slip length. The results are employed to propose a novel approach to directing bacterial motion on striped surfaces with different slip lengths, which implies a transformation of the circular motion into a snaking motion along the stripe boundaries. The feasibility of this approach is demonstrated by a simulation of active Brownian rods, which also reveals a dependence of directional motion on the stripe width.},
author = {Hu, Jinglei and Wysocki, Adam and Winkler, Roland G. and Gompper, Gerhard},
doi = {10.1038/srep09586},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/srep09586.pdf:pdf},
isbn = {2045-2322 (Electronic) 2045-2322 (Linking)},
issn = {2045-2322},
journal = {Sci. Rep.},
month = {aug},
number = {1},
pages = {9586},
pmid = {25993019},
title = {{Physical Sensing of Surface Properties by Microswimmers – Directing Bacterial Motion via Wall Slip}},
url = {http://www.nature.com/articles/srep09586},
volume = {5},
year = {2015}
}
@article{Yang2014,
abstract = {We simulate a model of self-propelled disks with soft repulsive interactions confined to a box in two dimensions. For small rotational diffusion rates, monodisperse disks spontaneously accumulate at the walls. At low densities, interaction forces between particles are strongly inhomogeneous, and a simple model predicts how these inhomogeneities alter the equation of state. At higher densities, collective effects become important. We observe signatures of a jamming transition at a packing fraction ϕ ∼ 0.88, which is also the jamming point for non-active athermal monodisperse disks. At this ϕ, the system develops a critical finite active speed necessary for wall aggregation. At packing fractions above ϕ ∼ 0.6, the pressure decreases with increasing density, suggesting that strong interactions between particles are affecting the equation of state well below the jamming transition. A mixture of bidisperse disks segregates in the absence of any adhesion, identifying a new mechanism that could contribute to cell sorting in embryonic development.},
archivePrefix = {arXiv},
arxivId = {1403.0697},
author = {Yang, Xingbo and Manning, M Lisa and Marchetti, M Cristina},
doi = {10.1039/c4sm00927d},
eprint = {1403.0697},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Soft Matter Volume 10 issue 34 2014 [doi 10.1039{\%}2Fc4sm00927d] Yang, Xingbo$\backslash$; Manning, M. Lisa$\backslash$; Marchetti, M. Cristina -- Aggregation and segregation of confined active particles.pdf:pdf},
isbn = {1744-683X},
issn = {1744-6848},
journal = {Soft Matter},
number = {34},
pages = {6477--6484},
pmid = {25046587},
title = {{Aggregation and segregation of confined active particles.}},
url = {http://pubs.rsc.org/en/content/articlehtml/2014/sm/c4sm00927d},
volume = {10},
year = {2014}
}
@article{Zottl2014,
abstract = {We study the collective motion of confined spherical microswimmers such as active colloids which we model by so-called squirmers. To simulate hydrodynamic flow fields including thermal noise, we use the method of multi-particle collision dynamics. We demonstrate that hydrodynamic near fields acting between squirmers as well as squirmers and bounding walls crucially determine their collective motion. In particular, with increasing density we observe a clear phase separation into a gas-like and cluster phase for neutral squirmers whereas strong pushers and pullers more gradually approach the hexagonal cluster state.},
archivePrefix = {arXiv},
arxivId = {1309.4352},
author = {Z{\"{o}}ttl, Andreas and Stark, Holger},
doi = {10.1103/PhysRevLett.112.118101},
eprint = {1309.4352},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1309.4352.pdf:pdf},
isbn = {0031-9007$\backslash$r1079-7114},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {11},
pages = {118101},
title = {{Hydrodynamics Determines Collective Motion and Phase Behavior of Active Colloids in Quasi-Two-Dimensional Confinement}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.118101},
volume = {112},
year = {2014}
}
@article{Jibuti2014,
abstract = {A three-dimensional model is proposed for Chlamydomonas Reinhardtii swimming with a breaststroke-like beating of its two flagella. The model reveals unusual angular orbits of the active swimmer under a linear shear flow. Namely, the swimmer sustains orientation transiently across the flow when flagella plane is perpendicular to the shear plane, and amplify the shear-induced rotation along the flow. Such behavior is a result of the interplay between shear-induced deformation and swimmer's periodic beating motion that exerts internal torques on the torque-free swimmer. This particular behavior has some significant consequences on the rheological properties of the suspension that tends to confirm previous experimental results [Phys. Rev. Lett. 104, 098102 (2010)]. We calculated the intrinsic viscosity of the suspension with such isolated modeled microswimmers (dilute case) in shear flow using numerical simulations based on Rotne-Prager approximation. The results show an increased intrinsic viscosity for active swimmer suspensions in comparison to non-active ones in accordance with previous experimental measurements. A major enhancement of the active swimmer viscosity occurs due to the effectively extended shape of the deformable swimming cells. We also recover the experimentally observed shear thinning behavior.},
archivePrefix = {arXiv},
arxivId = {1412.3176},
author = {Jibuti, Levan and Zimmermann, Walter and Rafa{\"{i}}, Salima and Peyla, Philippe},
eprint = {1412.3176},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1412.3176.pdf:pdf},
month = {dec},
pages = {8},
title = {{Effective viscosity of active suspensions: Three-dimensional numerical modeling}},
url = {http://arxiv.org/abs/1412.3176},
year = {2014}
}
@article{Awazu2014,
abstract = {We investigate the segregation pattern formations of strongly and weakly fluctuated Brownian particle mixtures, which are confined in spherical containers with finite volumes. We consider systems where the container restricts the motions of particles combining two familiar methods: spherically symmetric linear potential and the container edge wall. In such systems, the following two segregation patterns are observed. When the container radius is large enough, more weakly fluctuated particles accumulate around the center of the container than strongly fluctuated particles. On the other hand, inverted distributions of strongly and weakly fluctuated particles are observed when the container radius is small. We also found a similar segregation and phase inversion if such particle mixtures construct a chain (hetero-fluctuated polymer) and are confined in a container with no linear potential. We provide the qualitative mechanism and the relationships for the biopolymer behaviors of such phase inversions.},
archivePrefix = {arXiv},
arxivId = {1404.6405},
author = {Awazu, Akinori},
doi = {10.1103/PhysRevE.90.042308},
eprint = {1404.6405},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/Segregation and phase inversion of strongly and weakly ﬂuctuating Brownian particle mixtures.pdf:pdf},
isbn = {15393755},
issn = {1539-3755},
journal = {Phys. Rev. E},
month = {oct},
number = {4},
pages = {042308},
title = {{Segregation and phase inversion of strongly and weakly fluctuating Brownian particle mixtures and a chain of such particle mixtures in spherical containers}},
url = {https://link.aps.org/doi/10.1103/PhysRevE.90.042308},
volume = {90},
year = {2014}
}
@article{Peruani2012,
abstract = {We characterize cell motion in experiments and show that the transition to collective motion in colonies of gliding bacterial cells confined to a monolayer appears through the organization of cells into larger moving clusters. Collective motion by non-equilibrium cluster formation is detected for a critical cell packing fraction around 17{\%}. This transition is characterized by a scale-free power-law cluster size distribution, with an exponent {\$}0.88\backslashpm0.07{\$}, and the appearance of giant number fluctuations. Our findings are in quantitative agreement with simulations of self-propelled rods. This suggests that the interplay of self-propulsion of bacteria and the rod-shape of bacteria is sufficient to induce collective motion.},
archivePrefix = {arXiv},
arxivId = {1302.0311},
author = {Peruani, Fernando and Starruss, Joern and Jakovljevic, Vladimir and Sogaard-Andersen, Lotte and Deutsch, Andreas and Bar, Markus},
doi = {10.1103/PhysRevLett.108.098102},
eprint = {1302.0311},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1302.0311.pdf:pdf},
isbn = {0031-9007},
issn = {00319007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {9},
pages = {1--5},
pmid = {24312730},
title = {{Collective motion and nonequilibrium cluster formation in colonies of gliding bacteria}},
url = {http://arxiv.org/abs/1302.0311 http://dx.doi.org/10.1103/PhysRevLett.108.098102},
volume = {108},
year = {2013}
}
@article{Swiecicki2013,
abstract = {Escherichia coli swarmer cells coordinate their movement when confined in thin layers of fluid on agar surfaces. The motion and dynamics of cells, pairs of cells, and packs of cells can be recapitulated and studied in polymer microfluidic systems that are designed to constrain swarmer cell movement in thin layers of fluid between no-slip surfaces. The motion of elongated, smooth swimming E. coli cells in these environments reproduces the behavior of packs of cells observed at the leading edge of swarming communities and demonstrates the delicate balance between the physical dimensions of fluids and bacterial cell behavior.},
author = {Swiecicki, Jean-Marie and Sliusarenko, Olesksii and Weibel, Douglas B},
doi = {10.1039/c3ib40130h},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/nihms636178.pdf:pdf},
issn = {1757-9708},
journal = {Integr. Biol. (Camb).},
number = {12},
pages = {1490--4},
pmid = {24145500},
title = {{From swimming to swarming: Escherichia coli cell motility in two-dimensions.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/24145500{\%}5Cnhttp://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=PMC4222179},
volume = {5},
year = {2013}
}
@article{Abkenar2013,
abstract = {Collective behavior of self-propelled particles is observed on a microscale for swimmers such as sperm and bacteria as well as for protein filaments in motility assays. The properties of such systems depend both on their dimensionality and the interactions between their particles. We introduce a model for self-propelled rods in two dimensions that interact via a separation-shifted Lennard-Jones potential. Due to the finite potential barrier, the rods are able to cross. This model allows us to efficiently simulate systems of self-propelled rods that effectively move in two dimensions but can occasionally escape to the third dimension in order to pass each other. Our quasi-two-dimensional self-propelled particles describe a class of active systems that encompasses microswimmers close to a wall and filaments propelled on a substrate. Using Monte Carlo simulations, we first determine the isotropic-nematic transition for passive rods. Using Brownian dynamics simulations, we characterize cluster formation of self-propelled rods as a function of propulsion strength, noise, and energy barrier. Contrary to rods with an infinite potential barrier, an increase of the propulsion strength does not only favor alignment but also effectively decreases the potential barrier that prevents crossing of rods. We thus find a clustering window with a maximum cluster size at medium propulsion strengths.},
archivePrefix = {arXiv},
arxivId = {1309.2829},
author = {Abkenar, Masoud and Marx, Kristian and Auth, Thorsten and Gompper, Gerhard},
doi = {10.1103/PhysRevE.88.062314},
eprint = {1309.2829},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/Collective behavior of penetrable self-propelled rods in two dimensions.pdf:pdf},
issn = {15393755},
journal = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
number = {6},
pages = {1--11},
title = {{Collective behavior of penetrable self-propelled rods in two dimensions}},
volume = {88},
year = {2013}
}
@article{Reigh2012,
author = {Reigh, Shang Yik and Winkler, Roland G. and Gompper, Gerhard},
doi = {10.1039/c2sm07378a},
issn = {1744-683X},
journal = {Soft Matter},
number = {16},
pages = {4363},
title = {{Synchronization and bundling of anchored bacterial flagella}},
url = {http://xlink.rsc.org/?DOI=c2sm07378a},
volume = {8},
year = {2012}
}
@article{Babu2012a,
abstract = {The African trypanosome is a single flagellated micro-organism that causes the deadly sleeping$\backslash$n sickness in humans and animals. We study the locomotion of a model trypanosome by modeling the$\backslash$n spindle-shaped cell body using an elastic network of vertices with additional bending rigidity. The$\backslash$n flagellum firmly attached to the model cell body is either straight or helical. A bending wave$\backslash$n propagates along the flagellum and pushes the trypanosome forward in its viscous environment, which$\backslash$n we simulate with the method of multi-particle collision dynamics. The relaxation dynamics of the$\backslash$n model cell body due to a static bending wave reveals the sperm number from elastohydrodynamics as$\backslash$n the relevant parameter. Characteristic cell body conformations for the helically attached flagellum$\backslash$n resemble experimental observations. We show that the swimming velocity scales as the root of the$\backslash$n angular frequency of the bending wave reminiscent of predictions for an actuated slender rod$\backslash$n attached to a large viscous load. The swimming velocity for one geometry collapses on a single$\backslash$n master curve when plotted versus the sperm number. The helically attached flagellum leads to a$\backslash$n helical swimming path and a rotation of the model trypanosome about its long axis as observed in$\backslash$n experiments. The simulated swimming velocity agrees with the experimental value.},
author = {Babu, Sujin B. and Stark, Holger},
doi = {10.1088/1367-2630/14/8/085012},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Babu{\_}2012{\_}New{\_}J.{\_}Phys.{\_}14{\_}085012.pdf:pdf},
issn = {1367-2630},
journal = {New J. Phys.},
month = {aug},
number = {8},
pages = {085012},
title = {{Modeling the locomotion of the African trypanosome using multi-particle collision dynamics}},
url = {http://stacks.iop.org/1367-2630/14/i=8/a=085012?key=crossref.fafe4e2303cadd1ec43a522171cfae5b},
volume = {14},
year = {2012}
}
@article{Heddergott2012,
abstract = {Blood is a remarkable habitat: it is highly viscous, contains a dense packaging of cells and perpetually flows at velocities varying over three orders of magnitude. Only few pathogens endure the harsh physical conditions within the vertebrate bloodstream and prosper despite being constantly attacked by host antibodies. African trypanosomes are strictly extracellular blood parasites, which evade the immune response through a system of antigenic variation and incessant motility. How the flagellates actually swim in blood remains to be elucidated. Here, we show that the mode and dynamics of trypanosome locomotion are a trait of life within a crowded environment. Using high-speed fluorescence microscopy and ordered micro-pillar arrays we show that the parasites mode of motility is adapted to the density of cells in blood. Trypanosomes are pulled forward by the planar beat of the single flagellum. Hydrodynamic flow across the asymmetrically shaped cell body translates into its rotational movement. Importantly, the presence of particles with the shape, size and spacing of blood cells is required and sufficient for trypanosomes to reach maximum forward velocity. If the density of obstacles, however, is further increased to resemble collagen networks or tissue spaces, the parasites reverse their flagellar beat and consequently swim backwards, in this way avoiding getting trapped. In the absence of obstacles, this flagellar beat reversal occurs randomly resulting in irregular waveforms and apparent cell tumbling. Thus, the swimming behavior of trypanosomes is a surprising example of micro-adaptation to life at low Reynolds numbers. For a precise physical interpretation, we compare our high-resolution microscopic data to results from a simulation technique that combines the method of multi-particle collision dynamics with a triangulated surface model. The simulation produces a rotating cell body and a helical swimming path, providing a functioning simulation method for a microorganism with a complex swimming strategy.},
author = {Heddergott, Niko and Kr{\"{u}}ger, Timothy and Babu, Sujin B. and Wei, Ai and Stellamanns, Erik and Uppaluri, Sravanti and Pfohl, Thomas and Stark, Holger and Engstler, Markus},
doi = {10.1371/journal.ppat.1003023},
editor = {Beverley, Stephen M.},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PLoS Pathogens Volume 8 issue 11 2012 [doi 10.1371{\%}2Fjournal.ppat.1003023] Heddergott, Niko$\backslash$; Kr{\"{u}}ger, Timothy$\backslash$; Babu, Sujin B.$\backslash$; Wei, Ai$\backslash$; Ste -- Trypanosome Motion Represents an Adaptation to the Crowded.pdf:pdf},
isbn = {10.1371/journal.ppat.1003023},
issn = {1553-7374},
journal = {PLoS Pathog.},
month = {nov},
number = {11},
pages = {e1003023},
pmid = {23166495},
title = {{Trypanosome Motion Represents an Adaptation to the Crowded Environment of the Vertebrate Bloodstream}},
url = {http://dx.plos.org/10.1371/journal.ppat.1003023},
volume = {8},
year = {2012}
}
@incollection{Babu2012,
abstract = {The African trypanosome is a protozoan which causes sleeping sickness in mammals. To study the dynamics of this microorganismat low Reynolds number, we implement and investigate three swimmer models, the Taylor sheet, a constanttorque swimmer, and a model for the African trypanosome. The first two swimmers are based on a semi-flexible sheet and the third is a full three-dimensional model. We simulate the viscous fluid environment of the swimmers using a technique called multi-particle collision dynamics. We verify our technique by implementing the Taylor sheet which is activated by a bending wave traveling along the sheet. Its ballistic motion turns into diffusive motion when the sheet becomes passive. For the constant-torque swimmer we apply a torque to the semi-flexible sheet which assumes a cork-screw shape and then generates the thrust force for propelling the swimmer forward.Whereas the angular velocity scales linearly with the torque, the swimming velocity displays a non-linear dependence. Finally, our trypanosome model swims with the help of a beating flagellum attached to the cell body. Since it wraps around the body, the model trypanosome displays a helical swimming trajectory. The swimming velocity displays a non-linear increase with the beating frequency of the flagellum.},
address = {Berlin, Heidelberg},
author = {Babu, Sujin B and Schmeltzer, Christian and Stark, Holger},
doi = {10.1007/978-3-642-28302-4_2},
editor = {Tropea, Cameron and Bleckmann, Horst},
isbn = {978-3-642-28302-4},
pages = {25--41},
publisher = {Springer Berlin Heidelberg},
title = {{Swimming at Low Reynolds Number: From Sheets to the African Trypanosome BT - Nature-Inspired Fluid Mechanics: Results of the DFG Priority Programme 1207 ”Nature-inspired Fluid Mechanics” 2006-2012}},
url = {https://doi.org/10.1007/978-3-642-28302-4{\_}2},
year = {2012}
}
@article{Sokolov2012,
author = {Sokolov, Andrey and Aranson, Igor S.},
doi = {10.1103/PhysRevLett.109.248109},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Physical Review Letters Volume 109 issue 24 2012 [doi 10.1103{\%}2FPhysRevLett.109.248109] Sokolov, Andrey$\backslash$; Aranson, Igor S. -- Physical Properties of Collective Motion in Suspensions of Bacteria.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {24},
pages = {248109},
title = {{Physical Properties of Collective Motion in Suspensions of Bacteria}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.248109},
volume = {109},
year = {2012}
}
@article{Vicsek2012,
abstract = {We review the observations and the basic laws describing the essential aspects of collective motion - being one of the most common and spectacular manifestation of coordinated behavior. Our aim is to provide a balanced discussion of the various facets of this highly multidisciplinary field, including experiments, mathematical methods and models for simulations, so that readers with a variety of background could get both the basics and a broader, more detailed picture of the field. The observations we report on include systems consisting of units ranging from macromolecules through metallic rods and robots to groups of animals and people. Some emphasis is put on models that are simple and realistic enough to reproduce the numerous related observations and are useful for developing concepts for a better understanding of the complexity of systems consisting of many simultaneously moving entities. As such, these models allow the establishing of a few fundamental principles of flocking. In particular, it is demonstrated, that in spite of considerable differences, a number of deep analogies exist between equilibrium statistical physics systems and those made of self-propelled (in most cases living) units. In both cases only a few well defined macroscopic/collective states occur and the transitions between these states follow a similar scenario, involving discontinuity and algebraic divergences. {\textcopyright} 2012 Elsevier B.V.},
archivePrefix = {arXiv},
arxivId = {1010.5017},
author = {Vicsek, Tam{\'{a}}s and Zafeiris, Anna},
doi = {10.1016/j.physrep.2012.03.004},
eprint = {1010.5017},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1-s2.0-S0370157312000968-main.pdf:pdf},
isbn = {03701573},
issn = {03701573},
journal = {Phys. Rep.},
number = {3-4},
pages = {71--140},
pmid = {21620861},
title = {{Collective motion}},
volume = {517},
year = {2012}
}
@article{SRMcCandlish2012,
abstract = {We study mixtures of self-propelled and passive rod-like particles in two dimensions using Brown- ian dynamics simulations. The simulations demonstrate that the two species spontaneously segregate to generate a rich array of dynamical domain structures whose properties depend on the propulsion velocity, density, and composition. In addition to presenting phase diagrams as a function of the system parameters, we investigate the mechanisms driving segregation. We show that the difference in collision frequencies between self-propelled and passive rods provides a driving force for segregation, which is amplified by the tendency of the self-propelled rods to swarm or cluster. Finally, both self-propelled and passive rods exhibit giant number fluctuations for sufficient propulsion velocities.},
archivePrefix = {arXiv},
arxivId = {arXiv:1110.2479v2},
author = {SRMcCandlish},
doi = {10.1039/c2sm06960a},
eprint = {arXiv:1110.2479v2},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/C2SM06960A.pdf:pdf},
issn = {1744-683X},
journal = {Soft Matter},
number = {8},
pages = {2527},
title = {{Spontaneous segregation of self-propelled particles with different motilities}},
volume = {8},
year = {2012}
}
@article{Babu2011,
abstract = {The dynamics of a semi-flexible sheet or tethered membrane in a solvent is studied using the method of stochastic rotation dynamics. Hydrodynamic interactions between different parts of the sheet are naturally included in this method. We confirm the scaling law for the radius of gyration versus sheet size predicted for a self-avoiding tethered membrane. The mean-square displacement shows both sub-diffusive and diffusive behavior similar to linear polymers. In the intermediate scattering function the sub-diffusive behavior appears as stretched exponential which we reproduce in our simulations. Thereby, we confirm an early prediction between the roughness and the sub-diffusion exponent derived from Zimm dynamics (E. Frey, D.R. Nelson, J. Phys. I 1, 1715 (1991)). Finally, we show that the diffusion coefficient of the square sheet is inversely proportional to the edge length of the sheet again in good agreement with theoretical predictions.},
author = {Babu, S. B. and Stark, H.},
doi = {10.1140/epje/i2011-11136-2},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/The European Physical Journal E Volume 34 issue 12 2011 [doi 10.1140{\%}2Fepje{\%}2Fi2011-11136-2] S. B. Babu$\backslash$; H. Stark -- Dynamics of semi-flexible tethered sheets.pdf:pdf},
issn = {1292-895X},
journal = {Eur. Phys. J. E. Soft Matter},
month = {dec},
number = {12},
pages = {1--7},
pmid = {22197906},
title = {{Dynamics of semi-flexible tethered sheets : a simulation study using stochastic rotation dynamics.}},
url = {http://www.springerlink.com/index/10.1140/epje/i2011-11136-2 http://www.ncbi.nlm.nih.gov/pubmed/22197906},
volume = {34},
year = {2011}
}
@article{Chai2011,
abstract = {Bacteria often live in the form of surface-associated communities of cells termed biofilms. Within biofilms, there is a division of labor in which genetically identical cells differentiate to serve distinct functions. This cellular differentiation results from a response to extracellular signals that occur due to changes in the local environment of a cell or in response to signaling molecules that the cells themselves produce. In this review, we discuss differentiation in biofilms, focusing on the molecular mechanisms that regulate differentiation in the bacterium Bacillus subtilis. In this organism, there is a subpopulation of cells within a biofilm that produces a signal, while a different subpopulation of cells responds to it. Studying what signals cells use to communicate with each other within a biofilm will allow for better design of strategies to prevent and disrupt biofilms.},
author = {Chai, Liraz and Vlamakis, Hera and Kolter, Roberto},
doi = {10.1557/mrs.2011.68},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/MRS Bulletin Volume 36 issue 05 2011 [doi 10.1557{\%}2Fmrs.2011.68] Chai, Liraz$\backslash$; Vlamakis, Hera$\backslash$; Kolter, Roberto -- Extracellular signal regulation of cell differentiation in biofilms.pdf:pdf},
isbn = {0883-7694},
issn = {0883-7694},
journal = {MRS Bull.},
number = {05},
pages = {374--379},
title = {{Extracellular signal regulation of cell differentiation in biofilms}},
url = {http://www.journals.cambridge.org/abstract{\_}S0883769411000686{\%}5Cnpapers3://publication/doi/10.1557/mrs.2011.68},
volume = {36},
year = {2011}
}
@inproceedings{Aureli2017,
author = {Aureli, Matteo and Porfiri, Maurizio},
booktitle = {ASME 2011 Dyn. Syst. Control Conf. Bath/ASME Symp. Fluid Power Motion Control. Vol. 1},
doi = {10.1115/DSCC2011-6053},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/9{\_}1.pdf:pdf},
isbn = {978-0-7918-5475-4},
keywords = {DSCC2011-6053},
pages = {9--16},
publisher = {ASME},
title = {{A Model of Self-Propelled Particles Coordinating Under External Leadership}},
url = {http://proceedings.asmedigitalcollection.asme.org/proceeding.aspx?articleid=1638292},
year = {2011}
}
@article{Rafa??2010,
abstract = {The measurement of a quantitative and macroscopic parameter to estimate the global motility of a large population of swimming biological cells is a challenge. Experiments on the rheology of active suspensions have been performed. Effective viscosity of sheared suspensions of live unicellular motile microalgae (Chlamydomonas Reinhardtii) is far greater than for suspensions containing the same volume fraction of dead cells. In addition, suspensions show shear thinning behavior. We relate these macroscopic measurements to the orientation of individual swimming cells under flow and discuss our results in the light of several existing models.},
archivePrefix = {arXiv},
arxivId = {0909.4193},
author = {Rafa{\"{i}}, Salima and Jibuti, Levan and Peyla, Philippe},
doi = {10.1103/PhysRevLett.104.098102},
eprint = {0909.4193},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/0909.4193.pdf:pdf},
isbn = {0031-9007},
issn = {1079-7114},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {9},
pages = {098102},
pmid = {20367014},
title = {{Effective viscosity of microswimmer suspensions.}},
url = {http://arxiv.org/abs/0909.4193 http://dx.doi.org/10.1103/PhysRevLett.104.098102 http://www.ncbi.nlm.nih.gov/pubmed/20367014},
volume = {104},
year = {2010}
}
@article{Kearns2010,
abstract = {How bacteria regulate, assemble and rotate flagella to swim in liquid media is reasonably well understood. Much less is known about how some bacteria use flagella to move over the tops of solid surfaces in a form of movement called swarming. The focus of bacteriology is changing from planktonic to surface environments, and so interest in swarming motility is on the rise. Here, I review the requirements that define swarming motility in diverse bacterial model systems, including an increase in the number of flagella per cell, the secretion of a surfactant to reduce surface tension and allow spreading, and movement in multicellular groups rather than as individuals.},
archivePrefix = {arXiv},
arxivId = {NIHMS150003},
author = {Kearns, Daniel B},
doi = {10.1038/nrmicro2405},
eprint = {NIHMS150003},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/nrmicro2405.pdf:pdf},
isbn = {1740-1534 (Electronic)$\backslash$n1740-1526 (Linking)},
issn = {1740-1534},
journal = {Nat. Rev. Microbiol.},
keywords = {Bacteria,Bacteria: chemistry,Bacteria: cytology,Bacterial Physiological Phenomena,Flagella,Flagella: physiology,Movement},
number = {9},
pages = {634--44},
pmid = {20694026},
publisher = {Nature Publishing Group},
title = {{A field guide to bacterial swarming motility.}},
url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3135019{\&}tool=pmcentrez{\&}rendertype=abstract},
volume = {8},
year = {2010}
}
@article{Ramaswamy2010,
abstract = {Active particles contain internal degrees of freedom with the ability to take in and dissipate energy and, in the process, execute systematic movement. Examples include all living organisms and their motile constituents such as molecular motors. This article reviews recent progress in applying the principles of nonequilibrium statistical mechanics and hydrodynamics to form a systematic theory of the behavior of collections of active particles–active matter–with only minimal regard to microscopic details. A unified view of the many kinds of active matter is presented, encompassing not only living systems but inanimate analogs. Theory and experiment are discussed side by side.},
archivePrefix = {arXiv},
arxivId = {1004.1933},
author = {Ramaswamy, Sriram},
doi = {10.1146/annurev-conmatphys-070909-104101},
eprint = {1004.1933},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/annurev-conmatphys-070909-104101.pdf:pdf},
isbn = {1947-5454},
issn = {1947-5454},
journal = {Annu. Rev. Condens. Matter Phys.},
keywords = {bacterial motility,cell rheology,cytoskeleton,self-propulsion},
number = {1},
pages = {323--345},
pmid = {23688051},
title = {{The mechanics and statistics of active matter}},
url = {http://dx.doi.org/10.1146/annurev-conmatphys-070909-104101{\%}5Cnhttp://www.annualreviews.org/doi/10.1146/annurev-conmatphys-070909-104101},
volume = {1},
year = {2010}
}
@article{Damton2010,
abstract = {When vegetative bacteria that can swim are grown in a rich medium on an agar surface, they become multinucleate, elongate, synthesize large numbers of flagella, produce wetting agents, and move across the surface in coordinated packs: they swarm. We examined the motion of swarming Escherichia coli, comparing the motion of individual cells to their motion during swimming. Swarming cells' speeds are comparable to bulk swimming speeds, but very broadly distributed. Their speeds and orientations are correlated over a short distance (several cell lengths), but this correlation Is not isotropic. We observe the swirling that Is conspicuous in many swarming systems, probably due to increasingly long-lived correlations among cells that associate into groups. The normal run-tumble behavior seen in swimming chemotaxis is largely suppressed, instead, cells are continually reoriented by random jostling by their neighbors, randomizing their directions in a few tenths of a second. At the edge of the swarm, cells often pause, then swim back toward the center of the swarm or along its edge. Local alignment among cells, a necessary condition of many flocking theories, is accomplished by cell body collisions and/or shortrange hydrodynamic interactions. ?? 2010 by the Biophysical Society.},
author = {Damton, Nicholas C. and Turner, Linda and Rojevsky, Svetlana and Berg, Howard C.},
doi = {10.1016/j.bpj.2010.01.053},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/main.pdf:pdf},
isbn = {0006-3495},
issn = {00063495},
journal = {Biophys. J.},
number = {10},
pages = {2082--2090},
pmid = {20483315},
publisher = {Biophysical Society},
title = {{Dynamics of bacterial swarming}},
url = {http://dx.doi.org/10.1016/j.bpj.2010.01.053},
volume = {98},
year = {2010}
}
@article{Zhang2010,
abstract = {Flocking birds, fish schools, and insect swarms are familiar examples of collective motion that plays a role in a range of problems, such as spreading of diseases. Models have provided a qualitative understanding of the collective motion, but progress has been hindered by the lack of detailed experimental data. Here we report simultaneous measurements of the positions, velocities, and orientations as a function of time for up to a thousand wild-type Bacillus subtilis bacteria in a colony. The bacteria spontaneously form closely packed dynamic clusters within which they move cooperatively. The number of bacteria in a cluster exhibits a power-law distribution truncated by an exponential tail. The probability of finding clusters with large numbers of bacteria grows markedly as the bacterial density increases. The number of bacteria per unit area exhibits fluctuations far larger than those for populations in thermal equilibrium. Such "giant number fluctuations" have been found in models and in experiments on inert systems but not observed previously in a biological system. Our results demonstrate that bacteria are an excellent system to study the general phenomenon of collective motion.},
author = {Zhang, H P and Be'er, Avraham and Florin, E-L and Swinney, Harry L},
doi = {10.1073/pnas.1001651107},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PNAS-2010-Zhang-13626-30.pdf:pdf},
isbn = {1362613630},
issn = {1091-6490},
journal = {Proc. Natl. Acad. Sci. U. S. A.},
keywords = {Bacillus subtilis,Bacillus subtilis: cytology,Cluster Analysis,Microbial Viability,Models, Biological,Motion},
number = {31},
pages = {13626--30},
pmid = {20643957},
title = {{Collective motion and density fluctuations in bacterial colonies.}},
url = {http://www.pnas.org/cgi/content/long/107/31/13626},
volume = {107},
year = {2010}
}
@article{Yang2010,
abstract = {Systems of self-propelled particles are known for their tendency to aggregate and to display swarm behavior. We investigate two model systems, self-propelled rods interacting via volume exclusion, and sinusoidally-beating flagella embedded in a fluid with hydrodynamic interactions. In the flagella system, beating frequencies are Gaussian distributed with a non-zero average. These systems are studied by Brownian-dynamics simulations and by mesoscale hydrodynamics simulations, respectively. The clustering behavior is analyzed as the particle density and the environmental or internal noise are varied. By distinguishing three types of cluster-size probability density functions, we obtain a phase diagram of different swarm behaviors. The properties of clusters, such as their configuration, lifetime and average size are analyzed. We find that the swarm behavior of the two systems, characterized by several effective power laws, is very similar. However, a more careful analysis reveals several differences. Clusters of self-propelled rods form due to partially blocked forward motion, and are therefore typically wedge-shaped. At higher rod density and low noise, a giant mobile cluster appears, in which most rods are mostly oriented towards the center. In contrast, flagella become hydrodynamically synchronized and attract each other; their clusters are therefore more elongated. Furthermore, the lifetime of flagella clusters decays more quickly with cluster size than of rod clusters.},
archivePrefix = {arXiv},
arxivId = {1008.5309},
author = {Yang, Yingzi and Marceau, Vincent and Gompper, Gerhard},
doi = {10.1103/PhysRevE.82.031904},
eprint = {1008.5309},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/[I]Swarm behavior of self-propelled rods and swimming flagella Yingzi Gompper.pdf:pdf},
issn = {15393755},
journal = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
number = {3},
pages = {1--13},
pmid = {21230105},
title = {{Swarm behavior of self-propelled rods and swimming flagella}},
volume = {82},
year = {2010}
}
@article{Oberholzer2010,
abstract = {African trypanosomes are devastating human and animal pathogens that cause significant human mortality and limit economic development in sub-Saharan Africa. Studies of trypanosome biology generally consider these protozoan parasites as individual cells in suspension cultures or in animal models of infection. Here we report that the procyclic form of the African trypanosome Trypanosoma brucei engages in social behavior when cultivated on semisolid agarose surfaces. This behavior is characterized by trypanosomes assembling into multicellular communities that engage in polarized migrations across the agarose surface and cooperate to divert their movements in response to external signals. These cooperative movements are flagellum-mediated, since they do not occur in trypanin knockdown parasites that lack normal flagellum motility. We term this behavior social motility based on features shared with social motility and other types of surface-induced social behavior in bacteria. Social motility represents a novel and unexpected aspect of trypanosome biology and offers new paradigms for considering host-parasite interactions.},
author = {Oberholzer, Michael and Lopez, Miguel A. and McLelland, Bryce T. and Hill, Kent L.},
doi = {10.1371/journal.ppat.1000739},
editor = {Parsons, Marilyn},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/Social Motility in African Trypanosomes Michael{\_}PLOS{\_}2009.pdf:pdf},
isbn = {1553-7374 (Electronic)$\backslash$r1553-7366 (Linking)},
issn = {1553-7374},
journal = {PLoS Pathog.},
month = {jan},
number = {1},
pages = {e1000739},
pmid = {20126443},
title = {{Social Motility in African Trypanosomes}},
url = {http://dx.plos.org/10.1371/journal.ppat.1000739},
volume = {6},
year = {2010}
}
@article{Lauga2009,
abstract = {Cell motility in viscous fluids is ubiquitous and affects many biological processes, including reproduction, infection and the marine life ecosystem. Here we review the biophysical and mechanical principles of locomotion at the small scales relevant to cell swimming, tens of micrometers and below. At this scale, inertia is unimportant and the Reynolds number is small. Our emphasis is on the simple physical picture and fundamental flow physics phenomena in this regime. We first give a brief overview of the mechanisms for swimming motility, and of the basic properties of flows at low Reynolds number, paying special attention to aspects most relevant for swimming such as resistance matrices for solid bodies, flow singularities and kinematic requirements for net translation. Then we review classical theoretical work on cell motility, in particular early calculations of swimming kinematics with prescribed stroke and the application of resistive force theory and slender-body theory to flagellar locomotion. After examining the physical means by which flagella are actuated, we outline areas of active research, including hydrodynamic interactions, biological locomotion in complex fluids, the design of small-scale artificial swimmers and the optimization of locomotion strategies. (Some figures in this article are in colour only in the electronic version) This article was invited by Christoph Schmidt.},
archivePrefix = {arXiv},
arxivId = {0812.2887},
author = {Lauga, Eric and Powers, Thomas R},
doi = {10.1088/0034-4885/72/9/096601},
eprint = {0812.2887},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Lauga{\_}2009{\_}Rep.{\_}Prog.{\_}Phys.{\_}72{\_}096601.pdf:pdf},
isbn = {0034-4885},
issn = {0034-4885},
journal = {Rep. Prog. Phys. Rep. Prog. Phys},
number = {72},
pages = {96601--36},
pmid = {269292100002},
title = {{The hydrodynamics of swimming microorganisms}},
url = {http://iopscience.iop.org/0034-4885/72/9/096601},
volume = {72},
year = {2009}
}
@article{Sokolov2009,
abstract = {Measurements of the shear viscosity in suspensions of swimming Bacillus subtilis in free-standing liquid films have revealed that the viscosity can decrease by up to a factor of 7 compared to the viscosity of the same liquid without bacteria or with nonmotile bacteria. The reduction in viscosity is observed in two complementary experiments: one studying the decay of a large vortex induced by a moving probe and another measuring the viscous torque on a rotating magnetic particle immersed in the film. The viscosity depends on the concentration and swimming speed of the bacteria.},
author = {Sokolov, Andrey and Aranson, Igor S.},
doi = {10.1103/PhysRevLett.103.148101},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/PhysRevLett.103.148101.pdf:pdf},
issn = {00319007},
journal = {Phys. Rev. Lett.},
number = {14},
pages = {2--5},
pmid = {19905604},
title = {{Reduction of viscosity in suspension of swimming bacteria}},
volume = {103},
year = {2009}
}
@article{Copeland2009,
abstract = {Bacterial swarming is an example of dynamic self-assembly in microbiology in which the collective interaction of a population of bacterial cells leads to emergent behavior. Swarming occurs when cells interact with surfaces, reprogram their physiology and behavior, and adapt to changes in their environment by coordinating their growth and motility with other cells in the colony. This Review summarizes the salient biological and biophysical features of this system and describes our current understanding of swarming motility. We have organized this Review into four sections: (1) The biophysics and mechanisms of bacterial motility in fluids and its relevance to swarming. (2) The role of cell/molecule, cell/surface, and cell/cell interactions during swarming. (3) The changes in physiology and behavior that accompany swarming motility. (4) A concluding discussion of several interesting, unanswered questions that is particularly relevant to soft matter scientists.},
author = {Copeland, Matthew F. and Weibel, Douglas B.},
doi = {10.1039/b812146j},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/b812146j.pdf:pdf},
isbn = {1744-683X},
issn = {1744-683X},
journal = {Soft Matter},
number = {6},
pages = {1174},
pmid = {264099800007},
title = {{Bacterial swarming: a model system for studying dynamic self-assembly}},
url = {http://xlink.rsc.org/?DOI=b812146j},
volume = {5},
year = {2009}
}
@article{You2009,
abstract = {We present a particle-based simulation study on two-component swarms where there exist two different types of groups in a swarm. Effects of different parameters between the two groups are studied systematically based on Langevin's equation. It is shown that the mass difference can introduce a protective behavior for the lighter members of the swarm in a vortex state. When the self-propelling strength is allowed to differ between two groups, it is observed that the swarm becomes spatially segregated and finally separated into two components at a certain critical value. We also investigate effects of different preferences for shelters on their collective decision making. In particular, it is found that the probability of selecting a shelter from the other varies sigmoidally as a function of the number ratio. The model is shown to describe the dynamics of the shelter choosing process of the cockroach-robot mixed group satisfactorily. It raises the possibility that the present model can be applied to the problems of pest control and fishing using robots and decoys. ?? 2009 Elsevier Ltd. All rights reserved.},
author = {You, Sang Koo and Kwon, Dae Hyuk and ik Park, Yong and Kim, Sun Myong and Chung, Myung Hoon and Kim, Chul Koo},
doi = {10.1016/j.jtbi.2009.08.025},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1-s2.0-S0022519309004056-main.pdf:pdf},
isbn = {0022-5193},
issn = {00225193},
journal = {J. Theor. Biol.},
keywords = {Collective decision making,Collective motion,Multi-component swarm,Swarm dynamics},
number = {3},
pages = {494--500},
pmid = {19716374},
title = {{Collective behaviors of two-component swarms}},
volume = {261},
year = {2009}
}
@article{Gompper2009,
abstract = {In this review, we describe and analyze a mesoscale simulation method for fluid flow, which was introduced by Malevanets and Kapral in 1999, and is now called multi-particle collision dynamics (MPC) or stochastic rotation dynamics (SRD). The method consists of alternating streaming and collision steps in an ensemble of point particles. The multi-particle collisions are performed by grouping particles in collision cells, and mass, momentum, and energy are locally conserved. This simulation technique captures both full hydrodynamic interactions and thermal fluctuations. The first part of the review begins with a description of several widely used MPC algorithms and then discusses important features of the original SRD algorithm and frequently used variations. Two complementary approaches for deriving the hydrodynamic equations and evaluating the transport coefficients are reviewed. It is then shown how MPC algorithms can be generalized to model non-ideal fluids, and binary mixtures with a consolute point. The importance of angular-momentum conservation for systems like phase-separated liquids with different viscosities is discussed. The second part of the review describes a number of recent applications of MPC algorithms to study colloid and polymer dynamics, the behavior of vesicles and cells in hydrodynamic flows, and the dynamics of viscoelastic fluids.},
archivePrefix = {arXiv},
arxivId = {0808.2157},
author = {Gompper, G. and Ihle, T. and Kroll, D. M. and Winkler, R. G.},
doi = {10.1007/978-3-540-87706-6-1},
eprint = {0808.2157},
file = {:C$\backslash$:/Users/Adyant/Downloads/0808.2157.pdf:pdf},
isbn = {9783540877059},
issn = {00653195},
journal = {Adv. Polym. Sci.},
keywords = {Binary fluid mixtures,Colloids,Complex fluids,Hydrodynamics,Mesoscale simulation techniques,Microemulsions,Polymers,Red blood cells,Vesicles,Viscoelastic fluids},
number = {1},
pages = {1--87},
pmid = {23298332},
title = {{Multi-particle collision dynamics: A particle-based mesoscale simulation approach to the hydrodynamics of complex fluids}},
volume = {221},
year = {2009}
}
@article{Yang2008,
abstract = {Sperm swimming at low Reynolds number have strong hydrodynamic interactions when their concentration is high in vivo or near substrates in vitro. The beating tails not only propel the sperm through a fluid, but also create flow fields through which sperm interact with each other. We study the hydrodynamic interaction and cooperation of sperm embedded in a two-dimensional fluid by using a particle-based mesoscopic simulation method, multi-particle collision dynamics (MPC). We analyze the sperm behavior by investigating the relationship between the beating-phase difference and the relative sperm position, as well as the energy consumption. Two effects of hydrodynamic interaction are found, synchronization and attraction. With these hydrodynamic effects, a multi-sperm system shows swarm behavior with a power-law dependence of the average cluster size on the width of the distribution of beating frequencies.},
archivePrefix = {arXiv},
arxivId = {0810.4680},
author = {Yang, Yingzi and Elgeti, Jens and Gompper, Gerhard},
doi = {10.1103/PhysRevE.78.061903},
eprint = {0810.4680},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/[I]Cooperation of Sperm Yingzi Yang.pdf:pdf},
isbn = {1550-2376},
issn = {1539-3755},
journal = {Phys. Rev. E},
month = {dec},
number = {6},
pages = {061903},
pmid = {19256864},
title = {{Cooperation of sperm in two dimensions: Synchronization, attraction, and aggregation through hydrodynamic interactions}},
url = {https://link.aps.org/doi/10.1103/PhysRevE.78.061903},
volume = {78},
year = {2008}
}
@article{Wu2007,
abstract = {Many bacteria are able to spread rapidly over the surface using a strategy called swarming. When the cells cover a surface at high density and compete with each other for nutrients, swarming permits them to maintain rapid growth at the swarm edge. Swarming with flagella has been investigated for many years, and much has been learned about its regulation. Nevertheless, its choreography, which is somewhat related to the counterflow of pedestrians on a city sidewalk, has remained elusive. It is the bacterial equivalent of dancing toward the exit in a crowd of moving bodies that usually are in close contact. Myxococcus xanthus expands its swarms at 1.6 $\mu$m/min, about a third the speed of individual cells gliding over the same surface. Each cell has pilus engines at its front end and slime secretion engines at its rear. Using the known mechanics of these engines and the ways they are coordinated, we have developed a cell-based model to study the role of social interactions in bacterial swarming. The model is able to quantify the contributions of individual motility engines to swarming. It also shows that microscopic social interactions help to form the ordered collective motion observed in swarms.},
author = {Wu, Yilin and Jiang, Yi and Kaiser, Dale and Alber, Mark},
doi = {10.1371/journal.pcbi.0030253},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/journal.pcbi.0030253.PDF:PDF},
isbn = {1553-7358 (Electronic)},
issn = {1553734X},
journal = {PLoS Comput. Biol.},
number = {12},
pages = {2546--2558},
pmid = {18166072},
title = {{Social interactions in myxobacterial swarming}},
volume = {3},
year = {2007}
}
@article{Lauga2006,
abstract = {Near a solid boundary, Escherichia coli swims in clockwise circular motion. We provide a hydrodynamic model for this behavior. We show that circular trajectories are natural consequences of force-free and torque-free swimming and the hydrodynamic interactions with the boundary, which also leads to a hydrodynamic trapping of the cells close to the surface. We compare the results of the model with experimental data and obtain reasonable agreement. In particular, the radius of curvature of the trajectory is observed to increase with the length of the bacterium body.},
archivePrefix = {arXiv},
arxivId = {cond-mat/0506675},
author = {Lauga, Eric and DiLuzio, Willow R and Whitesides, George M and Stone, Howard A},
doi = {10.1529/biophysj.105.069401},
eprint = {0506675},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Biophysical Journal Volume 90 issue 2 2006 [doi 10.1529{\%}2Fbiophysj.105.069401] Lauga, Eric$\backslash$; DiLuzio, Willow R.$\backslash$; Whitesides, George M.$\backslash$; Stone, H -- Swimming in Circles- Motion of Bacteria near Solid Bo.pdf:pdf},
isbn = {0006-3495 (Print)$\backslash$r0006-3495 (Linking)},
issn = {0006-3495},
journal = {Biophys. J.},
keywords = {Algorithms,Bacteria,Bacteria: metabolism,Bacterial Adhesion,Bacterial Physiological Phenomena,Biophysics,Biophysics: methods,Cell Movement,Chemotaxis,Computer Simulation,Escherichia coli,Escherichia coli: metabolism,Flagella,Flagella: metabolism,Image Processing, Computer-Assisted,Microscopy, Phase-Contrast,Microscopy, Video,Models, Biological,Models, Statistical,Models, Theoretical,Motion,Movement},
number = {2},
pages = {400--12},
pmid = {16239332},
primaryClass = {cond-mat},
publisher = {Elsevier},
title = {{Swimming in circles: motion of bacteria near solid boundaries.}},
url = {http://www.sciencedirect.com/science/article/pii/S0006349506722214},
volume = {90},
year = {2006}
}
@article{Ishikawa2006,
abstract = {The interaction between two swimming Paramecium caudatum was investigated experimentally. Cell motion was restricted between flat plates, and avoiding and escape reactions were observed, as well as hydrodynamic interactions. The results showed that changes in direction between two swimming cells were induced mainly by hydrodynamic forces and that the biological reaction was a minor factor. Numerical simulations were also performed using a boundary element method. P. caudatum was modelled as a rigid spheroid with surface tangential velocity measured by a particle image velocimetry (PIV) technique. Hydrodynamic interactions observed in the experiment agreed well with the numerical simulations, so we can conclude that the present cell model is appropriate for describing the motion of P. caudatum.},
author = {Ishikawa, T and Hota, M},
doi = {10.1242/jeb.02537},
file = {:C$\backslash$:/Users/Adyant/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Ishikawa, Hota - 2006 - Interaction of two swimming Paramecia.pdf:pdf;:C$\backslash$:/Users/Adyant/Downloads/papers/Interaction of two swimming Paramecia.pdf:pdf},
issn = {0022-0949 (Print)$\backslash$r0022-0949 (Linking)},
journal = {J. Exp. Biol.},
keywords = {Animals,Escape Reaction,Locomotion,Mathematics,Models, Biological,Paramecium caudatum/*physiology},
number = {Pt 22},
pages = {4452--4463},
pmid = {17079716},
title = {{Interaction of two swimming Paramecia}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/17079716},
volume = {209},
year = {2006}
}
@article{Peruani2006,
abstract = {Motivated by aggregation phenomena in gliding bacteria, we study collective motion in a twodimensional model of active, self-propelled rods interacting through volume exclusion. In simulations with individual particles, we find that particle clustering is facilitated by a sufficiently large packing fraction (eta) or length-to-width ratio (kappa). The transition to clustering in simulations is well captured by a mean-field model for the cluster size distribution, which predicts that the transition values kappa{\_}c of the aspect ratio for a fixed packing fraction is given by kappa{\_}c = C/eta - 1 where C is a constant.},
archivePrefix = {arXiv},
arxivId = {cond-mat/0604490},
author = {Peruani, Fernando and Deutsch, Andreas and B{\"{a}}r, Markus},
doi = {10.1103/PhysRevE.74.030904},
eprint = {0604490},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/Nonequilibrium clustering of self-propelled rods.pdf:pdf},
isbn = {1539-3755},
issn = {15393755},
journal = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
number = {3},
pages = {1--4},
pmid = {17025586},
primaryClass = {cond-mat},
title = {{Nonequilibrium clustering of self-propelled rods}},
volume = {74},
year = {2006}
}
@article{DiLuzio2005,
abstract = {The motion of peritrichously flagellated bacteria close to surfaces is relevant to understanding the early stages of biofilm formation and of pathogenic infection. This motion differs from the random-walk trajectories of cells in free solution. Individual Escherichia coli cells swim in clockwise, circular trajectories near planar glass surfaces. On a semi-solid agar substrate, cells differentiate into an elongated, hyperflagellated phenotype and migrate cooperatively over the surface, a phenomenon called swarming. We have developed a technique for observing isolated E. coli swarmer cells moving on an agar substrate and confined in shallow, oxidized poly(dimethylsiloxane) (PDMS) microchannels. Here we show that cells in these microchannels preferentially 'drive on the right', swimming preferentially along the right wall of the microchannel (viewed from behind the moving cell, with the agar on the bottom). We propose that when cells are confined between two interfaces--one an agar gel and the second PDMS--they swim closer to the agar surface than to the PDMS surface (and for much longer periods of time), leading to the preferential movement on the right of the microchannel. Thus, the choice of materials guides the motion of cells in microchannels.},
author = {DiLuzio, Willow R and Turner, Linda and Mayer, Michael and Garstecki, Piotr and Weibel, Douglas B and Berg, Howard C. and Whitesides, George M},
doi = {10.1038/nature03660},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Nature Volume 435 issue 7046 2005 [doi 10.1038{\%}2Fnature03660] DiLuzio, Willow R.$\backslash$; Turner, Linda$\backslash$; Mayer, Michael$\backslash$; Garstecki, Pi -- Escherichia coli swim on the right-hand side.pdf:pdf},
isbn = {0028-0836},
issn = {0028-0836},
journal = {Nature},
number = {7046},
pages = {1271--1274},
pmid = {15988531},
title = {{Escherichia coli swim on the right-hand side.}},
volume = {435},
year = {2005}
}
@article{Huepe2004,
abstract = {Intermittent behavior is shown to appear in a system of self-driven interacting particles. In the ordered phase, most particles move in the same approximate direction, but the system displays a series of intermittent bursts during which the order is temporarily lost. This intermittency is characterized and its statistical properties are found analytically for a reduced system containing only two particles. For large systems, the particles aggregate into clusters that play an essential role in the intermittent dynamics. The study of the cluster statistics shows that both the cluster sizes and the transition probability between them follow power-law distributions. The exchange of particles between clusters is shown to satisfy detailed balance.},
author = {Huepe, Cristi{\'{a}}n and Aldana, Maximino},
doi = {10.1103/PhysRevLett.92.168701},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/PhysRevLett.92.168701.pdf:pdf},
isbn = {0031-9007 (Print)$\backslash$r0031-9007 (Linking)},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {apr},
number = {16},
pages = {168701},
pmid = {15169268},
title = {{Intermittency and Clustering in a System of Self-Driven Particles}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.92.168701},
volume = {92},
year = {2004}
}
@article{Lamura2001,
abstract = {A particle-based model for mesoscopic fluid dynamics is used to simulate steady and unsteady flows around a circular and a square cylinder in a two-dimensional channel for a range of Reynolds numbers between 10 and 130. Numerical results for the recirculation length, the drag coefficient, and the Strouhal number are reported and compared with previous experimental measurements and computational fluid dynamics data. The good agreement demonstrates the potential of this method for the investigation of complex flows.},
archivePrefix = {arXiv},
arxivId = {cond-mat/0110148},
author = {Lamura, A and Gompper, G and Ihle, T and Kroll, D. M},
doi = {10.1209/epl/i2001-00522-9},
eprint = {0110148},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/MPCD Flow around a circular and a square cylinder Lamura Gompper.pdf:pdf},
isbn = {0295-5075},
issn = {0295-5075},
journal = {Europhys. Lett.},
number = {3},
pages = {319--325},
primaryClass = {cond-mat},
title = {{Multi-particle collision dynamics: Flow around a circular and a square cylinder}},
url = {http://stacks.iop.org/0295-5075/56/i=3/a=319?key=crossref.29a6db78cdc6b006b4a25b199c236195},
volume = {56},
year = {2001}
}
@article{Malevanets1999,
abstract = {Complex fluids such as polymers in solution or multispecies reacting systems in fluid flows often can be studied only by employing a simplified description of the solvent motions. A stochastic model utilizing a synchronous, discrete-time dynamics with continuous ... $\backslash$n},
author = {Malevanets, Anatoly and Kapral, Raymond},
doi = {10.1063/1.478857},
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/mesosolv A. Malevanets .pdf:pdf},
isbn = {1041610205002},
issn = {0021-9606},
journal = {J. Chem. Phys.},
month = {may},
number = {17},
pages = {8605--8613},
pmid = {16185379},
title = {{Mesoscopic model for solvent dynamics}},
url = {http://aip.scitation.org/doi/10.1063/1.478857},
volume = {110},
year = {1999}
}
@article{Rauprich1996,
abstract = {Proteus mirabilis colonies exhibit striking geometric regularity. Basic microbiological methods and imaging techniques were used to measure periodic macroscopic events in swarm colony morphogenesis. We distinguished three initial phases (lag phase, first swarming phase, and first consolidation phase) followed by repeating cycles of subsequent swarming plus consolidation phases. Each Proteus swarm colony terrace corresponds to one swarming-plus-consolidation cycle. The duration of the lag phase was dependent upon inoculation density in a way that indicated the operation of both cooperative and inhibitory multicellular effects. On our standard medium, the second and subsequent swarm phases displayed structure in the form of internal waves visible with reflected and dark-field illumination. These internal waves resulted from organization of the migrating bacteria into successively thicker cohorts of swarmer cells. Bacterial growth and motility were independently modified by altering the composition of the growth medium. By varying the glucose concentration in the substrate, it was possible to alter biomass production without greatly affecting the kinetics of colony surface area expansion. By varying the agar concentration in the substrate, initial bacterial biomass production was unaffected but colony expansion dynamics were significantly altered. Higher agar concentrations led to slower, shorter swarm phases and longer consolidation phases. Thus, colony growth was restricted by higher agar concentrations but the overall timing of the swarming-plus-consolidation cycles remained constant. None of a variety of factors which had significant effects on colony expansion altered terracing frequencies at 32 degrees C, but the length of the swarming-plus-consolidation cycle was affected by temperature and medium enrichment. Some clinical isolates displayed significant differences in terracing frequencies at 32 degrees C. Our results defined a number of readily quantifiable parameters in swarm colony development. The data showed no connection between nutrient (glucose) depletion and the onset of different phases in swarm colony morphogenesis. Several observations point to the operation of density-dependent thresholds in controlling the transitions between distinct phases.},
author = {Rauprich, Oliver and Matsushita, Mitsugu and Weijer, Cornelis J. and Siegert, Florian and Esipov, Sergei E. and Shapiro, James A.},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1786525.pdf:pdf},
isbn = {0021-9193},
issn = {0021-9193},
journal = {J. Bacteriol.},
month = {nov},
number = {22},
pages = {6525--38},
pmid = {8932309},
title = {{Periodic phenomena in Proteus mirabilis swarm colony development.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/8932309 http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=PMC178539},
volume = {178},
year = {1996}
}
@article{Vicsek1995,
author = {Vicsek, Tam{\'{a}}s and Czir{\'{o}}k, Andr{\'{a}}s and Ben-Jacob, Eshel and Cohen, Inon and Shochet, Ofer},
doi = {10.1103/PhysRevLett.75.1226},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Vicsek{\_}SPP.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {aug},
number = {6},
pages = {1226--1229},
title = {{Novel Type of Phase Transition in a System of Self-Driven Particles}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.1226},
volume = {75},
year = {1995}
}
@article{Kamiya1987,
author = {Kamiya, Ritsu},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/1-s2.0-0014482787903570-main.pdf:pdf},
journal = {Cell},
pages = {299--304},
title = {{SHORT NOTE Intrinsic Difference in Beat Frequency between the Two Flagella of Chlamydomonas reinhardtii The unicellular alga Chlamydomonas swims with the two anterior flagella beating as in the breast stroke [ l-3 ]. The overall shape of the cell and the }},
year = {1987}
}
@article{,
file = {:E$\backslash$:/Adyant/Documents/Taylor Project/papers/Purcell{\_}life{\_}at{\_}low{\_}reynolds{\_}number.pdf:pdf},
number = {June 1976},
pages = {3--11},
title = {{No Title}},
volume = {45},
year = {1977}
}
@article{Hoeniger1964,
author = {Hoeniger, J. F. M.},
doi = {10.1139/m64-001},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Canadian Journal of Microbiology Volume 10 issue 1 1964 [doi 10.1139{\%}2Fm64-001] Hoeniger, J. F. M. -- CELLULAR CHANGES ACCOMPANYING THE SWARMING OF PROTEUS MIRABILIS- I. OBSERVATIONS OF LIVING CULTURE.pdf:pdf},
issn = {0008-4166},
journal = {Can. J. Microbiol.},
month = {feb},
number = {1},
pages = {1--9},
title = {{CELLULAR CHANGES ACCOMPANYING THE SWARMING OF PROTEUS MIRABILIS: I. OBSERVATIONS OF LIVING CULTURES}},
url = {http://www.nrcresearchpress.com/doi/abs/10.1139/m64-001},
volume = {10},
year = {1964}
}
@article{Maude1963,
author = {ROTHSCHILD},
doi = {10.1038/200381b0},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/Nature Volume 198 issue 4886 1963 [doi 10.1038{\%}2F1981221a0] ROTHSCHILD, -- Non-random Distribution of Bull Spermatozoa in a Drop of Sperm Suspension.pdf:pdf},
isbn = {0028-0836},
issn = {0028-0836},
journal = {Nature},
keywords = {CATTLE,EXPERIMENTAL LAB STUDY,PHYSIOLOGY,SPERMATOZOA},
month = {oct},
number = {4904},
pages = {381--381},
pmid = {14087906},
title = {{Non-random Distribution of Bull Spermatozoa in a Drop of Sperm Suspension}},
url = {http://www.nature.com/doifinder/10.1038/200381b0},
volume = {200},
year = {1963}
}
@article{Duncan1955,
author = {Duncan, Otis Dudley and Duncan, Beverly},
doi = {10.1086/221609},
file = {:C$\backslash$:/Users/Adyant/Downloads/papers/2772537.pdf:pdf},
issn = {0002-9602},
journal = {Am. J. Sociol.},
month = {mar},
number = {5},
pages = {493--503},
title = {{Residential Distribution and Occupational Stratification}},
url = {http://www.journals.uchicago.edu/doi/10.1086/221609},
volume = {60},
year = {1955}
}

